On Second-order Optimization Methods for Federated Learning

We consider federated learning (FL), where the training data is distributed across a large number of clients. The standard optimization method in this setting is Federated Averaging (FedAvg), which performs multiple local first-order optimization steps between communication rounds. In this work, we evaluate the performance of several second-order distributed methods with local steps in the FL setting which promise to have favorable convergence properties. We (i) show that FedAvg performs surprisingly well against its second-order competitors when evaluated under fair metrics (equal amount of local computations)-in contrast to the results of previous work. Based on our numerical study, we propose (ii) a novel variant that uses second-order local information for updates and a global line search to counteract the resulting local specificity.

==> giant.tex <==
\begin{algorithm}
    \begin{algorithmic}[h!]
    \WHILE{not converged}
        \STATE Send parameters $\weights^{t}$ to clients $\clients_\currentstep$
        \FOR{clients $\clients_\currentstep$ in parallel}
            \STATE Compute $\nabla f_\selectedclient(\weights)$
            \STATE Send $\nabla f_i(\weights)$ to server
        \ENDFOR
        \STATE $\nabla f(\weights) = \frac{1}{|\clients_\currentstep|} \sum_{i\in \clients_\currentstep} f_\selectedclient(\weights)$
        \STATE Send $\nabla f(\weights)$ to clients
        \FOR{clients $\clients_\currentstep$ in parallel}
                \STATE Solve $H_\selectedclient \update_\selectedclient = -\nabla f(\weights)$ for $\update_\selectedclient$ using CG-method
            \STATE Send $\gamma \update_\selectedclient$ to server
        \ENDFOR
        \STATE \textcolor{blue}{Discard all $\update_\selectedclient$ where CG didn't converge}
        \STATE \textcolor{blue}{Discard complete step when less than $\frac{1}{4}$ updates converged}
        \STATE $-H^{-1} \nabla f(\weights) 
        \approx -\frac{1}{|\clients_\currentstep|} \sum_{i\in \clients_\currentstep} H_\selectedclient^{-1} \nabla f(\weights) 
        = \update
        = \frac{1}{|\clients_\currentstep|} \sum_{i\in \clients_\currentstep} \update_\selectedclient$
        \STATE \textcolor{blue}{Choose new set $\clients_\currentstep$}
        \STATE Send $\update$ to clients
        \FOR{clients $\clients_\currentstep$ in parallel}
            \FOR{predefined step sizes $\stepsize_1, \ldots, \stepsize_l$}
                \STATE Compute $\func_i(\weights+\stepsize_m u)$
            \ENDFOR
            \STATE Send $\func_i(\weights+\stepsize_1 u), \ldots, \func_i(\weights+\stepsize_l u$ and $\func_i(\weights)$ to server
        \ENDFOR
        \STATE Find optimal stepsize $\stepsize$ with backtracking line search
        \STATE $w^{t+1} = w^{t} + \stepsize \update$
    \ENDWHILE
    \end{algorithmic}
\caption{GIANT and additions for \textcolor{blue}{federated learning} in blue}
\label{GIANT}
\end{algorithm}
